Deficit-Driven Stratified Acquisition for Building STRATA-S12: An Open SAR-Optical Corpus for Self-Supervised Learning

Building a co-registered SAR-optical corpus for self-supervised Earth Observation is above all an acquisition problem, yet the main multi-modal datasets are collected opportunistically, with no per-stratum quota control, so the regions and seasons that cloud cover hits hardest end up under-sampled. We present Deficit-Driven Stratified Acquisition (DDSA), an algorithm that casts the construction of a Sentinel-1/Sentinel-2 corpus as a constrained maximum-coverage problem over a land-cover-driven, hemisphere-corrected (class x season x region) stratification of target countries on all six inhabited continents, and solves it online: acquisition is ordered by marginal gain against a per-stratum deficit that the quality gates and a visual review of every accepted pair keep updating during the run. Three results follow from measuring the algorithm on its own product. First, stratum balance is a property of the deficit-driven ordering rather than of run length: replayed over all 2,928,370 real acquisition attempts, failures included, it populates all 192 strata within 0.05% of the attempts, against 4.03% for uniform round-robin effort and 20.5% for a random order. Second, whether a rejected attempt can be recovered is better predicted by how long its cause persists than by the type of defect: cloud rejections are recovered at eta = 18.8% against 41.4% for nodata, consistent with clouds persisting through a season. Third, the repair loop supplies 39.5% of the released pairs at no measurable quality cost, with 89.8% surviving manual review, but it adds yield rather than balance. The quality guarantee has a price: 2,928,370 acquisition attempts produced 740,746 released pairs. We release the corpus, STRATA-S12, with per-pair metadata sidecars aligned with the STAC and PDS4 standards and the FAIR principles, and a pre-registered linear probe confirms it is fit for self-supervised pre-training.

==> algo_evidence/tables/phaseC_table.tex <==
\begin{tabular}{l l r r r}
\toprule
Budget & Ordering & Strata covered & Min-fill & Norm.\ entropy \\
\midrule
5\% & deficit-greedy (Phase~C) & 192 & 7 & 0.996 \\
 & abundance-first & 2 & 0 & 0.130 \\
 & random & 192 & 0 & 0.904 \\
\midrule
25\% & deficit-greedy (Phase~C) & 192 & 7 & 0.982 \\
 & abundance-first & 12 & 0 & 0.463 \\
 & random & 192 & 2 & 0.904 \\
\midrule
100\% & deficit-greedy (Phase~C) & 192 & 7 & 0.904 \\
 & abundance-first & 192 & 7 & 0.904 \\
 & random & 192 & 7 & 0.904 \\
\bottomrule
\end{tabular}


==> reben/tables/probe_table.tex <==
% probe_table.tex - generado por master.py. Sin numeracion fija: LaTeX numera.
\begin{table}[t]
\centering
\caption{Frozen linear-probe performance on reBEN (BigEarthNet v2.0, 19-class multi-label), mean $\pm$ std over 3 seeds. The pre-registered criterion holds when $\mathrm{mean}_{pre}-\mathrm{std}_{pre}$ exceeds $\mathrm{mean}_{rnd}+\mathrm{std}_{rnd}$ on micro-mAP.}
\label{tab:probe}
\begin{tabular}{lcc}
\toprule
Metric & Pre-trained on $D$ & Random init \\
\midrule
micro-mAP (primary) & $0.5552 \pm 0.0022$ & $0.5158 \pm 0.0068$ \\
macro-mAP & $0.3366 \pm 0.0004$ & $0.2920 \pm 0.0046$ \\
\bottomrule
\end{tabular}
\end{table}

